The NNLO QCD soft function for 1-jettiness

We calculate the soft function for the global event variable 1-jettiness at next-to-next-to-leading order (NNLO) in QCD. We focus specifically on the non-Abelian contribution, which, unlike the Abelian part, is not determined by the next-to-leading order result. The calculation uses the known general forms for the emission of one and two soft partons and is performed using a sector-decomposition method that is spelled out in detail. Results are presented in the form of numerical fits to the 1-jettiness soft function for LHC kinematics (as a function of the angle between the incoming beams and the final-state jet) and for generic kinematics (as a function of three independent angles). These fits represent one of the needed ingredients for NNLO calculations that use the N-jettiness event variable to handle infrared singularities.

==> cases.tex <==
\section{Double real Phase space}


\color{blue}
Perform Sudakov expansion wrt to base vectors $i$ and $j$,
\beqn \label{ijphasespace}
PS^{(2)}(i,j)&=&\int \frac{d^d q_1}{(2 \pi)^{d-1}} \frac{d^d q_2}{(2 \pi)^{d-1}} 
\delta(q_1^2) \delta(q_2^2) \nonumber \\
&=&\frac{1}{2^8 \pi^4} \Big(\frac{(4 \pi)^\ep}{\Gamma(1-\ep)}\Big)^2 \Big(\frac{1}{\hs_{ij}}\Big)^{2-2\ep}
\int dq_1^i dq_1^j dq_2^i dq_2^j \Big(\frac{1}{q_1^i q_1^j q_2^i q_2^j}\Big)^\ep \nonumber \\
&\times& d\hat{\Omega}^{(1)}_{d-2}\, d\hat{\Omega}^{(2)}_{d-2} 
\eeqn
$d\hat{\Omega}^{(1)}_{d-2}$ is element of solid angle for 
particle 1 in $d-2$ dimensions, normalized so that it integrates to 1.
Let us choose vectors in the transverse plane given by
\beqn
\hp_{ij\,\perp}&=&\hp_{ij\,\perp} (1,0;0) \nonumber \\
q_{1\,\perp}&=&q_{1\,\perp}(\cos(\phiu),\sin(\phiu);0) \nonumber \\
q_{2\,\perp}&=&q_{2\,\perp}(\cos(\phid),\sin(\phid)\cos(\alphad);\sin(\phid) \sin(\alphad)\hat{n}_\ep)
\eeqn
Integrating over irrelevant angles we get,
\beq \label{SolidAngle}
\int d\hat{\Omega}^{(1)}_{d-2} d\hat{\Omega}^{(2)}_{d-2} =
 \int_0^\pi \frac{d \phiu}{N_{\phiu}} \sin^{-2 \ep}\phiu
         \int_0^\pi \frac{d \phid}{N_{\phid}} \sin^{-2 \ep}\phid
         \int_0^\pi \frac{d \alphad }{N_{\alphad }} \sin^{-1 -2 \ep}\alphad
\eeq
\beq
N_\alpha = -\frac{1}{\ep} \sqrt{\pi} \frac{\Gamma(1-\ep)}{\Gamma(\frac{1}{2}-\ep)},\;\;\;
N_\phi =4^\ep \pi \frac{\Gamma(1-2\ep)}{\Gamma(1-\ep)^2} = \sqrt{\pi} \frac{\Gamma(\frac{1}{2}-\ep)}{\Gamma(1-\ep)}
\eeq
\begin{equation} \label{BRR}
B_{RR} = \Big(\frac{e^{2 \ep \gamma_E}}{\Gamma(1-2 \ep)}\Big)
=1 - \frac{\pi^2}{3} \epsilon^2-\frac{8}{3} \zeta_3 \epsilon^3+\frac{\pi^4}{90} \epsilon^4 + O(\ep^5)
\end{equation}
It is worth noting that
\beq \label{Nidentity}
\frac{1}{N_\alpha N_\phi^2} = -\frac{\ep}{2^{2 \ep} \pi^2} \frac{\Gamma(1-\ep)^2}{\Gamma(1-2 \ep)}   = 
-\frac{\ep}{2^{2 \ep} \pi^2} 
\Big[\frac{\Gamma(1-\ep)}{(4 \pi)^\ep}\Big]^2\frac{B_{RR}}{S_\ep^2} 
\eeq
using definitions given in Eq.~(\ref{Sepdefinition}) and Eq.~(\ref{BRR}).
Exploiting rotational invariance we can write this as,
\beq \label{RotatedSolidAngle}
\int d\hat{\Omega}^{(1)}_{d-2} d\hat{\Omega}^{(2)}_{d-2} =
 \int_0^\pi \frac{d \phiu}{N_{\phiu}} \sin^{-2 \ep}\phiu
         \int_0^\pi \frac{d \phiud}{N_{\phiud}} \sin^{-2 \ep}\phiud
         \int_0^\pi \frac{d \alphaud }{N_{\alphaud }} \sin^{-1 -2 \ep}\alphaud
\eeq
where $\phiud$ and $\alphaud$ 
defined in a rotated frame
\beqn
\hp_{ij\,\perp}&=&\hp_{ij\,\perp} (\cos\phiu,-\sin\phiu;0) \nonumber \\
q_{1\,\perp}&=&q_{1\,\perp}(1,0;0) \nonumber \\
q_{2\,\perp}&=&q_{2\,\perp}(\cos(\phiud), \sin(\phiud)\cos(\alphaud);\sin(\phiud) \sin(\alphaud)\hat{n}_\ep)
\eeqn
and are implicitly defined by,
\beqn
\cos\phid&=& \cos\phiu \cos\phiud-\sin\phiu \sin\phiud\cos\alphaud  \\
\sin\alphad &=& \sin\phiud \sin\alphaud/\sin\phid 
\eeqn

Similiarly, in analogy with Eq.~(\ref{ijphasespace}) we can perform Sudakov expansion wrt to base vectors $i$ and $k$,
\beqn \label{ikphasespace}
PS^{(2)}(i,k)&=&\int \frac{d^d q_1}{(2 \pi)^{d-1}} \frac{d^d q_2}{(2 \pi)^{d-1}} 
\delta(q_1^2) \delta(q_2^2) \nonumber \\
&=&\frac{1}{2^8 \pi^4} \Big(\frac{(4 \pi)^\ep}{\Gamma(1-\ep)}\Big)^2 \Big(\frac{1}{\hs_{ik}}\Big)^{2-2\ep}
\int dq_1^i dq_1^k dq_2^i dq_2^k \Big(\frac{1}{q_1^i q_1^k q_2^i q_2^k}\Big)^\ep \nonumber \\
&\times& d\hat{\Omega}^{(1)}_{d-2}\, d\hat{\Omega}^{(2)}_{d-2} 
\eeqn

\subsection{Phase space case 1}

\subsubsection{Moved from earlier}

We now change variables so that, which appropriate when both $q_1^i,q_2^i$ are the smallest
\beq
q_1^i=\tauN \xi,\;
q_1^k=\frac{\tauN \xi}{s},\;
q_2^i=\tauN (1-\xi),\;
q_2^k=\frac{\tauN (1-\xi)}{t}
\eeq
\beqn \label{Twophasespacefinal}
&&\int PS^{(2)}(i,k) \delta(\tauN-q_1^i-q_2^i) = \nonumber \\
&&\frac{1}{2^8 \pi^4} \tauN^{3-4\ep} \Big(\frac{(4 \pi)^\ep}{\Gamma(1-\ep)}\Big)^2 \Big(\frac{1}{\hs_{ik}}\Big)^{2-2\ep}
\int d\xi ds dt (\xi (1-\xi))^{1-2 \ep} \frac{1}{s^{2-\ep} t^{2-\ep}} \nonumber \\
&\times& \int_0^\pi \frac{d \phiu}{N_{\phiu}} \sin^{-2 \ep}\phiu
\int_0^\pi \frac{d \phid }{N_{\phid}} \sin^{-2 \ep}\phid
\int_0^\pi \frac{d \beta}{N_{\beta}} \sin^{-1 -2 \ep}\beta
\eeqn
So rescaling the angular integrals we get, $\cos \beta = 1 - 2 x_\beta$
\beq
\int_0^\pi \, \frac{d \beta}{N_\beta} \, \sin^{-1-2\ep}\beta = 
 -\ep \frac{2 \Gamma(1-2 \ep)}{\Gamma(1-\ep)^2} \int_0^1 d x_\beta \,
x_\beta^{-1-\ep} (1-x_\beta)^{-1-\ep}
\eeq
So rescaling the angular integrals we get, $\phiu = \pi x_1$ 
\beq
\int_0^\pi \, \frac{d \phiu}{N_{\phiu}} \, \sin^{-2\ep}\phiu = 
\frac{\Gamma(1-\ep)^2}{4^\ep  \Gamma(1-2 \ep)} \int_0^1 \, d x_1 \, \sin^{-2\ep}(\pi x_1)
\eeq

\subsubsection{Original text}

Using Eq.~(\ref{ijphasespace}) to perform Sudakov expansion wrt to base vectors $i$ and $j$ 
we now change variables so that
\beq
q_1^i=\tauN \xi,\;
q_1^j=\frac{\tauN \xi}{s},\;
q_2^i=\tauN (1-\xi),\;
q_2^j=\frac{\tauN (1-\xi)}{t}
\eeq
The result is
\beqn \label{Twophasespacecase1}
&&\int PS^{(2)}(i,j) \delta(\tauN-q_1^i-q_2^i) \theta(q_1^j-q_1^i)\theta(q_1^k-q_1^i)\theta(q_2^j-q_2^i)\theta(q_2^k-q_2^i)
= \nonumber \\
&&\frac{1}{2^8 \pi^4} \tauN^{3-4\ep} \Big(\frac{(4 \pi)^\ep}{\Gamma(1-\ep)}\Big)^2 \Big(\frac{1}{\hs_{ij}}\Big)^{2-2\ep}
\int_0^1  d\xi ds dt (\xi (1-\xi))^{1-2 \ep} \frac{1}{s^{2-\ep} t^{2-\ep}} \nonumber \\
&\times& \int d\hat{\Omega}^{(1)}_{d-2}\, d\hat{\Omega}^{(2)}_{d-2} \;
\times \theta(A_{ij,k}(s,\cos\phi_{1k})-s)\theta(A_{ij,k}(t,\cos\phi_{2k})-t)
\eeqn
With no further transformation and using Eq.~(\ref{SolidAngle}) and Eq.~(\ref{Nidentity}) phase space becomes
\beqn \label{Twophasespacecase1untransformed}
&&\int PS^{(2)}(i,j) \delta(\tauN-q_1^i-q_2^j)
\theta(q_1^j-q_1^i)\theta(q_1^k-q_1^i)\theta(q_2^j-q_2^i)\theta(q_2^k-q_2^i) \nonumber \\
&&=-\frac{\ep}{2^{9+4\ep} \pi^4} \tauN^{3-4\ep} \frac{B_{RR}}{S_\ep^2} \Big(\frac{1}{\hs_{ij}}\Big)^{2-2\ep}
\int_0^1 d\xi ds dt (\xi (1-\xi))^{1-2 \ep} \frac{1}{s^{2-\ep} t^{2-\ep}} \nonumber \\
&\times& \int_0^1 d x_4 \; \sin^{-2 \ep}\phiu
         \int_0^1 d x_5 \; \sin^{-2 \ep}\phid
         \int_0^1 d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
&\times& \theta(A_{ij,k}(s,\cos\phi_{1k})-s)\theta(A_{ij,k}(t,\cos\phi_{2k})-t)
\eeqn
where $\phiu=\pi x_4,\phid=\pi x_5,\cos\alphad=1-2x_6$.

Denominators
\beqn \label{Denominators1}
2 \hp_i.q_1&=&\tauN \xi \nonumber \\
2 \hp_i.q_2&=&\tauN (1-\xi) \nonumber \\
2 \hp_j.q_1&=&\tauN \xi/s \nonumber \\
2 \hp_j.q_2&=&\tauN (1-\xi)/t \nonumber \\
2 q_1.q_2&=&\frac{1}{\hs_{ij}} \frac{\tauN^2 \xi  (1-\xi)}{s t} \Big[(\sqrt{s}-\sqrt{t})^2 +4 \zud \sqrt{s t}\Big],\;\;\zud=\frac{1}{2}(1-\cos\phiud)
\eeqn
where $\phiud$ is the angle between 1 and 2.
Map $\zud$ to a new variable $\lambda$ through the relation,
\beqn
\zud &=& \frac{ (\sqrt{s}-\sqrt{t})^2 (1-\lambda)}{(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}} \nonumber \\
1-\zud &=& \frac{ (\sqrt{s}+\sqrt{t})^2 \lambda}{(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}}
\eeqn
or the inverse,
\beqn
\lambda &=& \frac{(\sqrt{s}-\sqrt{t})^2\;(1-\zud)}{((\sqrt{s}-\sqrt{t})^2+4 \zud\sqrt{st} )}  \\
\lambda(1-\lambda)&=&\frac{((s-t)^2\;\zud (1-\zud)}{((\sqrt{s}-\sqrt{t})^2+4 \zud \sqrt{st} )^2}
\eeqn

So Jacobian of transformation from $\zud$ to $\lambda$ is, 
\beq
\frac{d \zud}{d \lambda} = -\frac{(s-t)^2}{[(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}]^2}
\eeq
In terms of the new variable $\lambda$ we have,
\beq \label{q1Dq2_transformed}
(\sqrt{s}-\sqrt{t})^2 +4 \zud \sqrt{st}
 = \frac{(s-t)^2}{(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}}
\eeq
so that
\beq
2 q_1.q_2 = \frac{1}{\hs_{ij}} \frac{\tauN^2 \xi(1-\xi)}{st}
 \frac{(s-t)^2}{(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}}
\eeq
%
Further
\beq
\sin^2 \phiud = 4 \zud (1-\zud)
 = 4 \frac{(s-t)^2 \lambda(1-\lambda)}{[(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}]^2}
\eeq
Part of the integrand that appears is given in Eq.~(\ref{RotatedSolidAngle})
\beqn \label{phiudintegral}
\int_0^\pi d\phiud \, \sin^{-2\ep}\phiud &=&
 \int_{-1}^1 d(\cos\phiud) \, [ \sin^2\phiud ]^{-\frac{1}{2}-\ep} 
 =2 \int_{0}^1 d\zud \left[ 4\zud(1-\zud) \right]^{-\frac{1}{2}-\ep} \nn \\
 &=& 2 \int_0^1 d\lambda \, \frac{d\zud}{d\lambda}  \left[ 4\zud(1-\zud) \right]^{-\frac{1}{2}-\ep} \nn \\
 &=& 2 \int_0^1 d\lambda \, \frac{(s-t)^2}{[(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}]^2}
  \left[ \frac{4(s-t)^2 \lambda(1-\lambda)}{[(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}]^2} \right]^{-\frac{1}{2}-\ep} \nn \\
 &=& 2^{-2\ep} \int_0^1 d\lambda \, \left[ \lambda(1-\lambda) \right]^{-\frac{1}{2}-\ep} 
  \, \frac{|s-t|^{1-2\ep}}{[(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}]^{1-2\ep}} \nn \\
 &=& 2^{-2\ep} \pi \int_0^1 dx_5 \, \left[ \lambda(1-\lambda) \right]^{-\ep} 
  \, \frac{|s-t|^{1-2\ep}}{[(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}]^{1-2\ep}} \nn \\
\eeqn
where $\lambda=\sin^2(\pi x_5/2)$.
Further we have that
\beq \label{alphaudintegral}
\int_0^\pi d \alphaud \, \sin^{-1-2\ep}\alphaud=\frac{1}{2^{1+2\ep}} \int_0^1 dx_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep}
\eeq
where $\cos \alphaud=1-2 x_6$.
Using Eq.~(\ref{RotatedSolidAngle}) we may show that the phase space becomes,
\beqn \label{Twophasespacecase1bis}
&&\int PS^{(2)}(i,j) \delta(\tauN-q_1^i-q_2^i) \theta(q_1^j-q_1^i)\theta(q_1^k-q_1^i)\theta(q_2^j-q_2^i)\theta(q_2^k-q_2^i)
= \nonumber \\
&&\frac{1}{2^{9+4\ep} \pi^2} \tauN^{3-4\ep} \Big(\frac{(4 \pi)^\ep}{\Gamma(1-\ep)}\Big)^2 \Big(\frac{1}{\hs_{ij}}\Big)^{2-2\ep}
\int_0^1  d\xi ds dt (\xi (1-\xi))^{1-2 \ep} \frac{1}{s^{2-\ep} t^{2-\ep}} \nonumber \\
&\times&\frac{1}{N_\phi^2 \, N_\alpha }\int_0^1 dx_4 \sin^{-2 \ep}\phiu
         \int_0^1 dx_5 \, (\lambda (1-\lambda))^{-\ep} \frac{|s-t|^{1-2\ep}}{[(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}]^{1-2\ep}} 
         \int_0^1 \, d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
&\times& \theta(A_{ij,k}(s,\cos\phi_{1k})-s)\theta(A_{ij,k}(t,\cos\phi_{2k})-t) \\
&=&\frac{1}{2^{9+6\ep} \pi^4} \tauN^{3-4\ep} \frac{B_{RR}}{S_\ep^2} \Big(\frac{1}{\hs_{ij}}\Big)^{2-2\ep}
\int_0^1  d\xi ds dt (\xi (1-\xi))^{1-2 \ep} \frac{1}{s^{2-\ep} t^{2-\ep}} \nonumber \\
&\times&\int_0^1 dx_4 \sin^{-2 \ep}\phiu
         \int_0^1 dx_5 \, (\lambda (1-\lambda))^{-\ep} \frac{|s-t|^{1-2\ep}}{[(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}]^{1-2\ep}}
         \times (-\ep) \int_0^1 \, d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
&\times& \theta(A_{ij,k}(s,\cos\phi_{1k})-s)\theta(A_{ij,k}(t,\cos\phi_{2k})-t)
\eeqn
where $\phi=\pi x_4$. For the last line we have exploited Eq.(\ref{Nidentity}).

Using the relations in Eq~(\ref{Denominators1}) and the transformation of Eq.~(\ref{q1Dq2_transformed}) we have,
\beqn 
|M^I|^2&=&
 g^4 S_\ep^2 \mu^{4 \ep} 
\frac{(-2) [\hp_i.q_1 \, \hp_j.q_2-\hp_j.q_1 \, \hp_i.q_2]^2}
     {q_1.q_2^2 \; \hp_i.(q_1+q_2)^2 \; \hp_j.(q_1+q_2)^2} \nonumber \\
  &=&-8 g^4 S_\ep^2 \mu^{4 \ep} \frac{\hs_{ij}^2}{\tauN^4} \, \frac{s^2 t^2}{[s-t]^2} \,
\frac{[(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}]^2}{[\xi t+(1-\xi)s]^2}  \\
|M^{II}|^2&=&g^4 S_\ep^2 \mu^{4 \ep} 
\frac{\hs_{ij}}{ q_1.q_2 \; \hp_i.(q_1+q_2) \; \hp_j.(q_1+q_2)} \nonumber \\
&=&8 g^4 S_\ep^2 \mu^{4 \ep} \frac{\hs_{ij}^2}{\tauN^4} \frac{s^2 t^2}{[s-t]^2} \frac{1}{\xi [1-\xi]} 
\frac{[(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}]}{[\xi t+(1-\xi)s]} \\
|M^{IIIa}|^2&=&8 g^4 S_\ep^2 \mu^{4 \ep} \frac{\hs_{ij}^2}{\tauN^4} \frac{s t}{\xi^2\; (1-\xi)^2}\\
|M^{IIIb}|^2&=&8 g^4 S_\ep^2 \mu^{4 \ep} \frac{\hs_{ij}^2}{\tauN^4} \frac{s^2t}{\xi\; (1-\xi)}
      \Big[-\frac{1}{2}\frac{1}{[\xi t+(1-\xi) s]}\Big] \\
|M^{IIIc}|^2&=&8 g^4 S_\ep^2 \mu^{4 \ep} \frac{\hs_{ij}^2}{\tauN^4} \frac{st^2}{\xi\; (1-\xi)}
      \Big[-\frac{1}{2}\frac{1}{[\xi t+(1-\xi) s]}\Big] \\
|M^{IIId}|^2&=&8 g^4 S_\ep^2 \mu^{4 \ep} \frac{\hs_{ij}^2}{\tauN^4} \frac{s t (s+t) }{\xi [1-\xi]} \Big(
     \frac{(t\; \Theta(s-t) +s\; \Theta(t-s))}{[\xi t+(1-\xi) s]} \frac{[(\sqrt{s}-\sqrt{t})^2+4 \lambda \sqrt{st}]}{(s-t)^2}\Big) \\
|M^{IIIe}|^2&=&8 g^4 S_\ep^2 \mu^{4 \ep} \frac{\hs_{ij}^2}{\tauN^4} \frac{s t (s+t)}{2 \xi [1-\xi]} \Big(
    \frac{(\Theta(s-t)-\Theta(t-s) }{[\xi t+(1-\xi) s]}
\frac{[(\sqrt{s}-\sqrt{t})^2+4 \lambda \sqrt{st}]}{(s-t)}\Big) \\
|M^{IIIf}|^2&=&-8 g^4 S_\ep^2 \mu^{4 \ep} \frac{\hs_{ij}^2}{\tauN^4}
     \frac{2 st}{ \xi^2 [1-\xi]^2}  \Big(
\frac{\big(t\; \Theta(s-t)+ s\; \Theta(t-s)\big )\; [(\sqrt{s}-\sqrt{t})^2+4 \lambda \sqrt{st}]}{(s-t)^2}\Big) \nonumber \\
\\
|M^{IIIg}|^2&=&-8 g^4 S_\ep^2 \mu^{4 \ep} \frac{\hs_{ij}^2}{\tauN^4}
\frac{st}{\xi^2 [1-\xi]^2} \;
\Big( \frac{(\Theta(s-t)-\Theta(t-s)) \; [(\sqrt{s}-\sqrt{t})^2+4 \lambda \sqrt{st}]}{(s-t)}\Big) \nonumber \\
\eeqn
Combining phase space Eq.(\ref{Twophasespacecase1}) and matrix element we have, ***These need to be updated***
\beqn
I^{(2),ii,I}_{q\bar{q},ij} &=& -\cN_{ij} 2^{-6\ep} B_{RR} 
\int_0^1  d\xi ds dt (\xi (1-\xi))^{1-2 \ep} \; (st)^{\ep} |s-t|^{-1-2\ep}\nonumber \\
&\times&\int_0^1 dx_4 \sin^{-2 \ep}\phiu
         \int_0^1 dx_5 \, (\lambda (1-\lambda))^{-\ep} 
         \times (-\ep) \int_0^1 \, d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
&\times& \frac{[(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}]^{1+2 \ep}}
 {[\xi t +(1-\xi) s ]^2}\nonumber \\
&\times& \theta(A_{ij,k}(s,\cos\phi_{1k})-s)\theta(A_{ij,k}(t,\cos\phi_{2k})-t) \\
I^{(2),ii,II}_{q\bar{q},ij} &=& \cN_{ij} 2^{-6\ep} B_{RR}
\int_0^1  d\xi ds dt (\xi (1-\xi))^{-2 \ep} \; (st)^{\ep} |s-t|^{-1-2\ep}\nonumber \\
&\times&\int_0^1 dx_4 \sin^{-2 \ep}\phiu
         \int_0^1 dx_5 \, (\lambda (1-\lambda))^{-\ep} 
         \times (-\ep) \int_0^1 \, d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
&\times& \frac{[(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}]^{2 \ep}}
 {[\xi t +(1-\xi) s ]}\nonumber \\
&\times& \theta(A_{ij,k}(s,\cos\phi_{1k})-s)\theta(A_{ij,k}(t,\cos\phi_{2k})-t) \\
I^{(2),ii,IIIc}_{q\bar{q},ij} &=& \cN_{ij} 2^{-6\ep} B_{RR}
\int_0^1  d\xi ds dt (\xi (1-\xi))^{-2 \ep} \; (st)^{-1+\ep}(s+t)^2 |s-t|^{-1-2\ep}\nonumber \\
&\times&\int_0^1 dx_4 \sin^{-2 \ep}\phiu
         \int_0^1 dx_5 \, (\lambda (1-\lambda))^{-\ep} 
         \times (-\ep) \int_0^1 \, d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
&\times& \frac{[(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}]^{2 \ep}}
 {2\; [\xi t +(1-\xi) s ]}\nonumber \\
&\times& \theta(A_{ij,k}(s,\cos\phi_{1k})-s)\theta(A_{ij,k}(t,\cos\phi_{2k})-t) \\
I^{(2),ii,IIId}_{q\bar{q},ij} &=& -\cN_{ij} 2^{-6\ep} B_{RR}
\int_0^1  d\xi ds dt (\xi (1-\xi))^{-1-2 \ep} \; (s+t) (st)^{-1+\ep} |s-t|^{-1-2\ep}\nonumber \\
&\times&\int_0^1 dx_4 \sin^{-2 \ep}\phiu
         \int_0^1 dx_5 \, (\lambda (1-\lambda))^{-\ep} 
         \times (-\ep) \int_0^1 \, d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
&\times& [(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}]^{2 \ep} \nonumber \\
&\times& \theta(A_{ij,k}(s,\cos\phi_{1k})-s)\theta(A_{ij,k}(t,\cos\phi_{2k})-t)
\eeqn
where
\beq \label{Normalizationdefinition}
\cN_{ij}=\Big(\frac{\as}{2 \pi}\Big)^2 \, \frac{1}{\tauN} \, \Big[\frac{\tauN}{\mu \sqrt{\hs_{ij}}}\Big]^{-4\ep}
\eeq
with $B_{RR}$ given by Eq.~(\ref{BRR}).
Combining phase space Eq.(\ref{Twophasespacecase1untransformed}) and matrix element we have,
\beqn
I^{(2),ii,IIIa}_{q\bar{q},ij} &=&  \cN_{ij} 2^{-4\ep} B_{RR}
\int_0^1  d\xi ds dt (\xi (1-\xi))^{-1-2 \ep} \; (st)^{-1+\ep} \nonumber \\
&\times& \int_0^1 d x_4 \; \sin^{-2 \ep}\phiu
         \int_0^1 d x_5 \; \sin^{-2 \ep}\phid
         \times (-\ep) \int_0^1 d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
&\times& \theta(A_{ij,k}(s,\cos\phi_{1k})-s)\theta(A_{ij,k}(t,\cos\phi_{2k})-t) \\
I^{(2),ii,IIIb}_{q\bar{q},ij} &=& \cN_{ij} 2^{-4\ep} B_{RR}
\int_0^1  d\xi ds dt (\xi (1-\xi))^{-2 \ep} \; (s^{-1+\ep} t^{\ep}+s^{\ep} t^{-1+\ep}) \nonumber \\
&\times& \int_0^1 d x_4 \; \sin^{-2 \ep}\phiu
         \int_0^1 d x_5 \; \sin^{-2 \ep}\phid
         \times (-\ep) \int_0^1 d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
&\times& \Big[\frac{-1}{2[\xi t+(1-\xi) s]}\Big] \;
\theta(A_{ij,k}(s,\cos\phi_{1k})-s)\theta(A_{ij,k}(t,\cos\phi_{2k})-t)
\eeqn
\subsection{Phase space case 2}
Using Eq.~(\ref{ijphasespace}) to perform Sudakov expansion wrt to base vectors $i$ and $j$ 
we now change variables so that
\beq
q_1^i=\tauN \xi,\;
q_1^j=\frac{\tauN \xi}{s},\;
q_2^j=\tauN (1-\xi),\;
q_2^i=\frac{\tauN (1-\xi)}{t}
\eeq
\beqn \label{Twophasespacecase2}
&&\int PS^{(2)}(i,j) \delta(\tauN-q_1^i-q_2^j)
\theta(q_1^j-q_1^i)\theta(q_1^k-q_1^i)\theta(q_2^i-q_2^j)\theta(q_2^k-q_2^j) \nonumber \\
&&\frac{1}{2^8 \pi^4} \tauN^{3-4\ep} \Big(\frac{(4 \pi)^\ep}{\Gamma(1-\ep)}\Big)^2 \Big(\frac{1}{\hs_{ij}}\Big)^{2-2\ep}
\int_0^1 d\xi ds dt (\xi (1-\xi))^{1-2 \ep} \frac{1}{s^{2-\ep} t^{2-\ep}} \nonumber \\
&\times& \int d\hat{\Omega}^{(1)}_{d-2}\, d\hat{\Omega}^{(2)}_{d-2} \;
\times \theta(A_{ij,k}(s,\cos\phi_{1k})-s)\theta(A_{ji,k}(t,\cos\phi_{2k})-t)
\eeqn
Denominators
\beqn \label{Denominators2}
2 \hp_i.q_1&=&\tauN \xi \nonumber \\
2 \hp_j.q_1&=&\tauN \xi/s \nonumber \\
2 \hp_i.q_2&=&\tauN (1-\xi)/t \nonumber \\
2 \hp_j.q_2&=&\tauN (1-\xi) \nonumber \\
2 q_1.q_2&=&\frac{\tauN^2 \xi  (1-\xi)}{s t \hs_{ij}} \Big[(1-\sqrt{st})^2 +4 \zud \sqrt{s t}\Big],\;\;\zud=\frac{1}{2}(1-\cos\phiud)
\eeqn
Using Eq.~(\ref{RotatedSolidAngle}) and Eq.~(\ref{Nidentity}) phase space becomes
\beqn
&&\int PS^{(2)}(i,j) \delta(\tauN-q_1^i-q_2^j)
\theta(q_1^j-q_1^i)\theta(q_1^k-q_1^i)\theta(q_2^i-q_2^j)\theta(q_2^k-q_2^j) \nonumber \\
&&=-\frac{\ep}{2^{9+4\ep} \pi^4} \tauN^{3-4\ep} \frac{B_{RR}}{S_\ep^2} \Big(\frac{1}{\hs_{ij}}\Big)^{2-2\ep}
\int_0^1 d\xi ds dt (\xi (1-\xi))^{1-2 \ep} \frac{1}{s^{2-\ep} t^{2-\ep}} \nonumber \\
&\times& \int_0^1 d x_4 \; \sin^{-2 \ep}\phiu
         \int_0^1 d x_5 \; \sin^{-2 \ep}\phid
         \int_0^1 d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
&\times& \theta(A_{ij,k}(s,\cos\phi_{1})-s)\theta(A_{ji,k}(t,\cos\phi_{2})-t)
\eeqn
where $\phiu=\pi x_4,\phid=\pi x_5,\cos\alphad=1-2x_6, \zud=\frac{1}{2}(1-\cos\phiud)$, and
\beq
\cos\phiud=\cos\phiu \cos\phid +\sin\phiu \sin\phid\cos\alphad 
\eeq

Using the relations in Eq~(\ref{Denominators2}) the matrix element is given by,
\beqn 
|M^I|^2&=&
 g^4 S_\ep^2 \mu^{4 \ep} 
\frac{(-2) [\hp_i.q_1 \, \hp_j.q_2-\hp_j.q_1 \, \hp_i.q_2]^2}
     {q_1.q_2^2 \; \hp_i.(q_1+q_2)^2 \; \hp_j.(q_1+q_2)^2} \nonumber \\
  &=&-8 g^4 S_\ep^2 \mu^{4 \ep} \frac{\hs_{ij}^2}{\tauN^4} \, 
    \frac{s^2 \; t^2 \; (1-st)^2} {[(1-\sqrt{st})^2+4 \zud\sqrt{st}]^2 \; [\xi t+(1-\xi)]^2 \; [\xi+(1-\xi) s]^2} \\
|M^{II}|^2&=&g^4 S_\ep^2 \mu^{4 \ep} 
\frac{\hs_{ij}}{ q_1.q_2 \; \hp_i.(q_1+q_2) \; \hp_j.(q_1+q_2)} \nonumber \\
&=&8 g^4 S_\ep^2 \mu^{4 \ep} \frac{\hs_{ij}^2}{\tauN^4} \frac{s^2 t^2}{\xi(1-\xi)} 
\frac{1}{[(1-\sqrt{st})^2+4 \zud\sqrt{st}] \; [\xi t+(1-\xi)] \; [\xi+(1-\xi) s]} \\
|M^{III}|^2 &=&8 g^4 S_\ep^2 \mu^{4 \ep} \frac{\hs_{ij}^2}{\tauN^4} \frac{s t}{\xi(1-\xi)} \nonumber \\ 
  &\times&\Big[\frac{1}{\xi\;(1-\xi)} \Big(1-\frac{1-st}{[(1-\sqrt{st})^2+4 \zud\sqrt{st}]}\Big) \nonumber \\ 
  &+&\frac{1}{2} \frac{(1+st)^2}{[(1-\sqrt{st})^2+4 \zud\sqrt{st}]\; \; [\xi t+(1-\xi)] \; [\xi+(1-\xi)s]} \nonumber \\ 
  &-&\frac{1}{2} \frac{(1+st)}{[\xi t+(1-\xi)] \; [\xi+(1-\xi)s]} \Big]
%Id,ansIII=8g^4*Sep^2*pow(mu,4*ep)*sij^2/tauN^4*s*t/xi/[1-xi]*(
%      +xi^-1*[1-xi]^-1*(1-(1+s*t)/[(1-rts*rtt)^2+4*z12*rts*rtt])
%      +1/2*(1+s*t)^2/[(1-rts*rtt)^2+4*z12*rts*rtt]/[xi*t+(1-xi)]/[xi+(1-xi)*s]
%      -1/2/[xi*t+(1-xi)]/[xi+(1-xi)*s]*(1+s*t)
\eeqn
Combining phase space and matrix element we have,
\beqn
I^{(2),ij,I}_{q\bar{q},ij} &=& -\cN_{ij} 2^{-4\ep} B_{RR} 
\int_0^1  d\xi ds dt (\xi (1-\xi))^{1-2 \ep} \; (st)^{\ep} (1-s t)^{2}\nonumber \\
&\times&\int_0^1 dx_4 \sin^{-2 \ep}\phiu
         \int_0^1 dx_5 \sin^{-2 \ep}\phid
         \times (-\ep) \int_0^1 \, d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
&\times& \frac{1}{[(1-\sqrt{st})^2 +4 \zud \sqrt{st}]^2\; [\xi t +(1-\xi) ]^2 \; [\xi +(1-\xi) s ]^2}\nonumber \\
&\times& \theta(A_{ij,k}(s,\cos\phi_{1k})-s)\theta(A_{ij,k}(t,\cos\phi_{2k})-t) \\
I^{(2),ij,II}_{q\bar{q},ij} &=& \cN_{ij} 2^{-4\ep} B_{RR}
\int_0^1  d\xi ds dt (\xi (1-\xi))^{-2 \ep} \; (st)^{\ep} \nonumber \\
 &\times & \int_0^1 dx_4 \sin^{-2 \ep}\phiu  \; \int_0^1 dx_5 \sin^{-2 \ep}\phid
         \times (-\ep) \int_0^1 \, d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
&\times& \frac{1}{[(1-\sqrt{st})^2 +4 \zud \sqrt{st}]\; [\xi t +(1-\xi) ]\, [\xi +(1-\xi) s ]}\nonumber \\
&\times& \theta(A_{ij,k}(s,\cos\phi_{1k})-s)\theta(A_{ij,k}(t,\cos\phi_{2k})-t) \\
I^{(2),ij,IIIa}_{q\bar{q},ij} &=& \cN_{ij} 2^{-4\ep} B_{RR}
\int_0^1  d\xi ds dt (\xi (1-\xi))^{-1-2 \ep} \; (st)^{-\frac{1}{2}+\ep} \nonumber \\
 &\times & \int_0^1 dx_4 \sin^{-2 \ep}\phiu  \; \int_0^1 dx_5 \sin^{-2 \ep}\phid
         \times (-\ep) \int_0^1 \, d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
&\times& \frac{-2(1-2z_{12})}{[(1-\sqrt{st})^2+4 \zud\sqrt{st}]}  \nonumber \\
&\times&\theta(A_{ij,k}(s,\cos\phi_{1k})-s)\theta(A_{ij,k}(t,\cos\phi_{2k})-t) \\
I^{(2),ij,IIIb}_{q\bar{q},ij} &=& \cN_{ij} 2^{-4\ep} B_{RR}
\int_0^1  d\xi ds dt (\xi (1-\xi))^{-2 \ep} \; (st)^{-\frac{1}{2}+\ep} \nonumber \\
 &\times & \int_0^1 dx_4 \sin^{-2 \ep}\phiu  \; \int_0^1 dx_5 \sin^{-2 \ep}\phid
         \times (-\ep) \int_0^1 \, d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
  &\times &\frac{(1+st)(1-2z_{12})}{[(1-\sqrt{st})^2+4 \zud\sqrt{st}]\; \; [\xi t+(1-\xi)] \; [\xi+(1-\xi)s]} \nonumber \\ 
  &\times &\theta(A_{ij,k}(s,\cos\phi_{1k})-s)\theta(A_{ij,k}(t,\cos\phi_{2k})-t) \nonumber \\
\eeqn
where $\cN$ is defined in Eq.~(\ref{Normalizationdefinition}).
\subsection{Phase space case 3}
Using Eq.~(\ref{ikphasespace}), to perform Sudakov expansion wrt to base vectors $i$ and $k$ 
we now change variables so that
\beq
q_1^i=\tauN \xi,\;
q_1^k=\frac{\tauN \xi}{s},\;
q_2^k=\tauN (1-\xi),\;
q_2^i=\frac{\tauN (1-\xi)}{t}
\eeq
\beqn \label{Twophasespacecase3}
&&\int PS^{(2)}(i,k) \delta(\tauN-q_1^i-q_2^k)\theta(q_1^j-q_1^i)\theta(q_1^k-q_1^i)\theta(q_2^i-q_2^k)\theta(q_2^j-q_2^k) = \nonumber \\
&&\frac{1}{2^8 \pi^4} \tauN^{3-4\ep} \Big(\frac{(4 \pi)^\ep}{\Gamma(1-\ep)}\Big)^2 \Big(\frac{1}{\hs_{ik}}\Big)^{2-2\ep}
\int_0^1 d\xi ds dt (\xi (1-\xi))^{1-2 \ep} \frac{1}{s^{2-\ep} t^{2-\ep}} \nonumber \\
&\times& \int d\hat{\Omega}^{(1)}_{d-2}\, d\hat{\Omega}^{(2)}_{d-2} \;
\times \theta(A_{ik,j}(s,\cos\phi_{1j})-s)\theta(A_{ki,j}(t,\cos\phi_{2j})-t)
\eeqn
Denominators
\beqn \label{Denominators3}
2 \hp_i.q_1&=&\tauN \xi \nonumber \\
2 \hp_i.q_2&=&\tauN (1-\xi)/t \nonumber \\
2 \hp_k.q_1&=&\tauN \xi/s \nonumber \\
2 \hp_k.q_2&=&\tauN (1-\xi) \nonumber \\
2 \hp_j.q_1&=&\frac{\tauN \xi}{s} \, A_{ik,j}(s,\cos(\phi_{j1})  \nonumber \\
2 \hp_j.q_2&=&\frac{\tauN (1-\xi)}{t} \, A_{ki,j}(t,\cos(\phi_{j2})  \nonumber \\
2 q_1.q_2&=&\frac{\tauN^2 \xi  (1-\xi)}{s t \hs_{ik}} \Big[(1-\sqrt{st})^2 +4 \zud \sqrt{s t}\Big],\;\;\zud=\frac{1}{2}(1-\cos\phiud)
\eeqn

Using Eq.~(\ref{RotatedSolidAngle}) and Eq.~(\ref{Nidentity}) phase space becomes
\beqn
&&\int PS^{(2)}(i,k) \delta(\tauN-q_1^i-q_2^k)
\theta(q_1^j-q_1^i)\theta(q_1^k-q_1^i)\theta(q_2^i-q_2^k)\theta(q_2^j-q_2^k) \nonumber \\
&&=-\frac{\ep}{2^{9+4\ep} \pi^4} \tauN^{3-4\ep} \frac{B_{RR}}{S_\ep^2} \Big(\frac{1}{\hs_{ik}}\Big)^{2-2\ep}
\int_0^1 d\xi ds dt (\xi (1-\xi))^{1-2 \ep} \frac{1}{s^{2-\ep} t^{2-\ep}} \nonumber \\
&\times& \int_0^1 d x_4 \; \sin^{-2 \ep}\phiu
         \int_0^1 d x_5 \; \sin^{-2 \ep}\phid
         \int_0^1 d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
&\times& \theta(A_{ik,j}(s,\cos\phi_{1j})-s)\theta(A_{ki,j}(t,\cos\phi_{2j})-t)
\eeqn
where $\phiu=\pi x_4,\phid=\pi x_5,\cos\alphad=1-2x_6, \zud=\frac{1}{2}(1-\cos\phiud)$, and
\beq
\cos\phiud=\cos\phiu \cos\phid +\sin\phiu \sin\phid\cos\alphad 
\eeq

Using the relations in Eq~(\ref{Denominators3}) the matrix element is given by,
\beqn 
|M^I|^2&=&
 g^4 S_\ep^2 \mu^{4 \ep} 
\frac{(-2) [\hp_i.q_1 \, \hp_j.q_2-\hp_j.q_1 \, \hp_i.q_2]^2}
     {q_1.q_2^2 \; \hp_i.(q_1+q_2)^2 \; \hp_j.(q_1+q_2)^2} 
  =-8 g^4 S_\ep^2 \mu^{4 \ep} \frac{\hs_{ik}^2}{\tauN^4} 
 \frac{s^2 \; t^4}{[(1-\sqrt{st})^2+4 \zud\sqrt{st}]^2} \nonumber \\
 &\times& \frac{[A_{ik,j}(s,\cos\phiu)-A_{ki,j}(t,\cos\phid) s]^2}
 {[\xi t A_{ik,j}(s,\cos\phiu)+(1-\xi) s A_{ki,j}(t,\cos\phid)]^2 \; [\xi t+(1-\xi)]^2 } \\
|M^{II}|^2&=&g^4 S_\ep^2 \mu^{4 \ep} 
\frac{\hs_{ij}}{ q_1.q_2 \; \hp_i.(q_1+q_2) \; \hp_j.(q_1+q_2)} 
=8 g^4 S_\ep^2 \mu^{4 \ep} \frac{\hs_{ij}\hs_{ik}}{\tauN^4} \frac{s^2 t^3}{\xi(1-\xi)} \nonumber \\
&\times& \frac{1}{[(1-\sqrt{st})^2+4 \zud\sqrt{st}] \; [\xi t A_{ik,j}(s,\cos\phiu)+(1-\xi) s A_{ki,j}(t,\cos\phid)] \; [\xi t+(1-\xi)]} \\
|M^{IIIa}|^2&=&8 g^4 S_\ep^2 \mu^{4 \ep}   \frac{\hs_{ij}\hs_{ik}}{\tauN^4} \frac{s t^2}{\xi^2(1-\xi)^2} \nonumber \\
&\times& \Bigg\{ 
 \Bigg(\frac{\hs_{ij}}{\hs_{ik}}-\frac{\Big(A_{ik,j}(s,\cos\phiu)+s A_{ki,j}(t,\cos\phid)\Big)}{((1-\sqrt{st})^2+4\zud \sqrt{st})}\Bigg) 
           \frac{1}{A_{ik,j}(s,\cos\phiu)\; A_{ki,j}(t,\cos\phid)} \Bigg\} \\
|M^{IIIb}|^2&=&8 g^4 S_\ep^2 \mu^{4 \ep}   \frac{\hs_{ij}\hs_{ik}}{\tauN^4} \frac{s t^2}{\xi(1-\xi)} \nonumber \\
&\times& \Bigg\{
      \frac{t}{[\xi t A_{ik,j}(s,\cos\phiu)+(1-\xi) s A_{ki,j}(t,\cos\phid)]\; [(1-\sqrt{st})^2+4 \zud \sqrt{st}]\;(\xi t+(1-\xi))} \nonumber \\
     &\times& \frac{1}{2} \Big(\sqrt{\frac{A_{ik,j}(s,\cos\phiu)}{A_{ki,j}(t,\cos\phid)}}
                            +s \sqrt{\frac{A_{ki,j}(t,\cos\phid)}{A_{ik,j}(s,\cos\phiu)}}\Big)^2 \nonumber \\       
     &-& \frac{1}{2} \frac{\hs_{ij}}{\hs_{ik}} \frac{t}{(\xi t A_{ik,j}(s,\cos\phiu)+(1-\xi) s A_{ki,j}(t,\cos\phid) \; (\xi t+(1-\xi))} \nonumber \\           
     &\times&  \Bigg(\frac{1}{A_{ki,j}(t,\cos\phid)}+\frac{s}{A_{ik,j}(s,\cos\phiu)}\Bigg)
\Bigg\}
\eeqn
%
%Id,ansI= -8*g^4*Sep^2*pow(mu,4*ep)*sik^2/tauN^4*s^2*t^4
%   *(Aikj(s,coshphi1)-Akij(t,coshphi2)*s)^2
%  /[(1-rts*rtt)^2+4*z12*rts*rtt]^2
%  /[xi*t*Aikj(s,coshphi1)+(1-xi)*s*Akij(t,coshphi2)]^2/[xi*t+(1-xi)]^2
% ;
%Id,ansII=+8*g^4*Sep^2*pow(mu,4*ep)*sij*sik/tauN^4*s^2*t^3/xi/[1-xi]
%  /[(1-rts*rtt)^2+4*z12*rts*rtt]/[xi*t*Aikj(s,coshphi1)+(1-xi)*s*Akij(t,coshphi2)]/[xi*t+(1-xi)];
%
%Id,ansIII=+8*g^4*Sep^2*pow(mu,4*ep)*sij*sik/tauN^4*s*t^2/xi/[1-xi]*(
%       + 1/xi/[1-xi]*(1/[(1-rts*rtt)^2+4*z12*rts*rtt]
%        *(-1/[Akij(t,coshphi2)]-s/[Aikj(s,coshphi1)])
%       + sij/sik/[Aikj(s,coshphi1)]/[Akij(t,coshphi2)])
%
%       +t/[xi*t*Aikj(s,coshphi1)+(1-xi)*s*Akij(t,coshphi2)]/[(1-rts*rtt)^2+4*z12*rts*rtt]/[xi*t+(1-xi)]
%        *1/2*(sqrt(Aikj(s,coshphi1))*invsqrt([Akij(t,coshphi2)])+s*sqrt(Akij(t,coshphi2))*invsqrt([Aikj(s,coshphi1)]))^2
%       -1/2*sij/sik*t/[xi*t*Aikj(s,coshphi1)+(1-xi)*s*Akij(t,coshphi2)]/[xi*t+(1-xi)]
%         *(1/[Akij(t,coshphi2)]+s/[Aikj(s,coshphi1)])
%          );
Combining phase space and matrix element we have,
\beqn
I^{(2),ij,I}_{q\bar{q},ik} &=& -\cN_{ij} 2^{-4\ep} \big(\frac{\hs_{ik}}{\hs_{ij}}\big)^{2\ep}\; B_{RR} 
\int_0^1  d\xi ds dt (\xi (1-\xi))^{1-2 \ep} \; s^{\ep}\; t^{2+\ep} \nonumber \\
&\times&\int_0^1 dx_4 \sin^{-2 \ep}\phiu
         \int_0^1 dx_5 \sin^{-2 \ep}\phid
         \times (-\ep) \int_0^1 \, d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
&\times& \frac{[A_{ik,j}(s,\cos\phiu)-A_{ki,j}(t,\cos\phid) s]^2}{[(1-\sqrt{s t})^2 +4 \zud \sqrt{st}]^2\; [\xi t A_{ik,j}(s,\cos\phiu)+(1-\xi) s A_{ki,j}(t,\cos\phid)]^2\; [\xi t +(1-\xi) ]^2 }\nonumber \\
&\times& \theta(A_{ij,k}(s,\cos\phi_{1k})-s)\theta(A_{ij,k}(t,\cos\phi_{2k})-t) \\
I^{(2),ij,II}_{q\bar{q},ik} &=& \cN_{ij} 2^{-4\ep} \big(\frac{\hs_{ik}}{\hs_{ij}}\big)^{2\ep}B_{RR} \frac{\hs_{ij}}{\hs_{ik}}
\int_0^1  d\xi ds dt (\xi (1-\xi))^{-2 \ep} \; s^{\ep} \; t^{1+\ep} 
\nonumber \\
 &\times & \int_0^1 dx_4 \sin^{-2 \ep}\phiu  \; \int_0^1 dx_5 \sin^{-2 \ep}\phid
         \times (-\ep) \int_0^1 \, d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
&\times& \frac{1}{[(1-\sqrt{st})^2 +4 \zud \sqrt{st}]\; \; [\xi t A_{ik,j}(s,\cos\phiu)+(1-\xi) s A_{ki,j}(t,\cos\phid)] \; [\xi t +(1-\xi) ]}\nonumber \\
&\times& \theta(A_{ij,k}(s,\cos\phi_{1k})-s)\theta(A_{ij,k}(t,\cos\phi_{2k})-t) \nonumber \\
I^{(2),ij,IIIa}_{q\bar{q},ik} &=& \cN_{ij} 2^{-4\ep} \big(\frac{\hs_{ik}}{\hs_{ij}}\big)^{2\ep}B_{RR} \frac{\hs_{ij}}{\hs_{ik}}
\int_0^1  d\xi ds dt (\xi (1-\xi))^{-1-2 \ep} \; s^{-1+\ep} \; t^{\ep} 
\nonumber \\
 &\times & \int_0^1 dx_4 \sin^{-2 \ep}\phiu  \; \int_0^1 dx_5 \sin^{-2 \ep}\phid
         \times (-\ep) \int_0^1 \, d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
&\times& \Bigg\{ 
 \Bigg(\frac{\hs_{ij}}{\hs_{ik}}-\frac{\Big(A_{ik,j}(s,\cos\phiu)+s A_{ki,j}(t,\cos\phid)\Big)}{((1-\sqrt{st})^2+4\zud \sqrt{st})}\Bigg) 
           \frac{1}{A_{ik,j}(s,\cos\phiu)\; A_{ki,j}(t,\cos\phid)} \Bigg\} \nonumber \\
&\times& \theta(A_{ij,k}(s,\cos\phi_{1k})-s)\theta(A_{ij,k}(t,\cos\phi_{2k})-t) \\
I^{(2),ij,IIIb}_{q\bar{q},ik} &=& \cN_{ij} 2^{-4\ep} \big(\frac{\hs_{ik}}{\hs_{ij}}\big)^{2\ep}B_{RR}
\int_0^1  d\xi ds dt (\xi (1-\xi))^{-2 \ep} \; s^{-1+\ep} \; t^{\ep} 
\nonumber \\
 &\times & \int_0^1 dx_4 \sin^{-2 \ep}\phiu  \; \int_0^1 dx_5 \sin^{-2 \ep}\phid
         \times (-\ep) \int_0^1 \, d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
 &\times& \frac{\hs_{ij}}{\hs_{ik}} \frac{t}{2}
   \frac{A_{ik,j}(s,\cos\phiu) +s A_{ki,j}(t,\cos\phid)}{A_{ik,j}(s,\cos\phiu) \, A_{ki,j}(t,\cos\phid) \,
   [\xi t A_{ik,j}(s,\cos\phiu)+(1-\xi) s A_{ki,j}(t,\cos\phid)] \, (\xi t+(1-\xi))} \nonumber \\
 &\times& \Bigg\{
      \frac{\left(A_{ik,j}(s,\cos\phiu) +s A_{ki,j}(t,\cos\phid)\right)}{[(1-\sqrt{st})^2+4 \zud \sqrt{st}]}
       - \frac{\hs_{ij}}{\hs_{ik}} \Bigg\} \nonumber \\
&\times& \theta(A_{ij,k}(s,\cos\phi_{1k})-s)\theta(A_{ij,k}(t,\cos\phi_{2k})-t)
\eeqn
where $\cN$ is defined in Eq.~(\ref{Normalizationdefinition}).
\subsection{Phase space case 4}
Using Eq.~(\ref{ikphasespace}), perform Sudakov expansion wrt to base vectors $i$ and $k$
we now change variables so that
\beq
q_1^k=\tauN \xi,\;
q_1^i=\frac{\tauN \xi}{s},\;
q_2^k=\tauN (1-\xi),\;
q_2^i=\frac{\tauN (1-\xi)}{t}
\eeq
\beqn \label{Twophasespacecase4}
&&\int PS^{(2)}(i,k) \delta(\tauN-q_1^k-q_2^k) \theta(q_1^i-q_1^k)\theta(q_1^j-q_1^k)\theta(q_2^i-q_2^k)\theta(q_2^j-q_2^k) \nonumber \\
&=&\frac{1}{2^8 \pi^4} \tauN^{3-4\ep} \Big(\frac{(4 \pi)^\ep}{\Gamma(1-\ep)}\Big)^2 \Big(\frac{1}{\hs_{ik}}\Big)^{2-2\ep}
\int_0^1 d\xi ds dt (\xi (1-\xi))^{1-2 \ep} \frac{1}{s^{2-\ep} t^{2-\ep}} \nonumber \\
&\times& \int d\hat{\Omega}^{(1)}_{d-2}\, d\hat{\Omega}^{(2)}_{d-2} \;
\times \theta(A_{ki,j}(s,\cos\phi_{1j})-s)\theta(A_{ki,j}(t,\cos\phi_{2j})-t)
\eeqn
By analogy with Eq.~(\ref{Twophasespacecase1bis}) this can be written as
\beqn
&&\int \int PS^{(2)}(i,k) \delta(\tauN-q_1^k-q_2^k) \theta(q_1^i-q_1^k)\theta(q_1^j-q_1^k)\theta(q_2^i-q_2^k)\theta(q_2^j-q_2^k) \nonumber \\
&=&\frac{1}{2^{9+6\ep} \pi^4} \tauN^{3-4\ep} \frac{B_{RR}}{S_\ep^2} \Big(\frac{1}{\hs_{ik}}\Big)^{2-2\ep}
\int_0^1  d\xi ds dt (\xi (1-\xi))^{1-2 \ep} \frac{1}{s^{2-\ep} t^{2-\ep}} \nonumber \\
&\times&\int_0^1 dx_4 \sin^{-2 \ep}\phiu
         \int_0^1 dx_5 \, (\lambda (1-\lambda))^{-\ep} \frac{|s-t|^{1-2\ep}}{[(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}]^{1-2\ep}}
         \times (-\ep) \int_0^1 \, d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
&\times& \theta(A_{ki,j}(s,\cos\phi_{1j})-s)\theta(A_{ki,j}(t,\cos\phi_{2j})-t)
\eeqn
Denominators
\beqn
2 \hp_i.q_1&=&\tauN \xi/s \nonumber \\
2 \hp_i.q_2&=&\tauN (1-\xi)/t \nonumber \\
2 \hp_j.q_1&=&\frac{\tauN \xi }{s} \, A_{ki,j}(s,\cos(\phi_{1j}))  \nonumber \\
2 \hp_j.q_2&=&\frac{\tauN (1-\xi)}{t} \, A_{ki,j}(t,\cos(\phi_{2j}))  \nonumber \\
2 q_1.q_2&=&\frac{\tauN^2 \xi  (1-\xi)}{s t \hs_{ik}} \Big[(\sqrt{s}-\sqrt{t})^2 +4 \zud \sqrt{s t}\Big],\;\;\zud=\frac{1}{2}(1-\cos\phiud)
\eeqn
\beqn 
|M^I|^2&=&
 g^4 S_\ep^2 \mu^{4 \ep} 
\frac{(-2) [\hp_i.q_1 \, \hp_j.q_2-\hp_j.q_1 \, \hp_i.q_2]^2}
     {q_1.q_2^2 \; \hp_i.(q_1+q_2)^2 \; \hp_j.(q_1+q_2)^2} 
  = -8 g^4 S_\ep^2 \mu^{4 \ep} \frac{\hs_{ik}^2}{\tauN^4} \, \frac{s^4 t^4}{[s-t]^4} \nonumber \\
&\times& \Bigg[\frac{[ A_{ki,j}(s,\cos\phi_{1j})- A_{ki,j}(t,\cos\phi_{2j})]\; [(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}]}
 {[\xi t A_{ki,j}(s,\cos\phi_{1j})+(1-\xi) s A_{ki,j}(t,\cos\phi_{2j})]\;[\xi t+(1-\xi)s]}\Bigg]^2 \\
\label{MsqII-case4}
|M^{II}|^2&=&g^4 S_\ep^2 \mu^{4 \ep} \frac{\hs_{ij}}{ q_1.q_2 \; \hp_i.(q_1+q_2) \; \hp_j.(q_1+q_2)} 
   = 8 g^4 S_\ep^2 \mu^{4 \ep} \frac{\hs_{ij} \hs_{ik} }{\tauN^4} \frac{s^3 t^3}{[s-t]^2} \frac{1}{\xi (1-\xi)} \nonumber \\
&\times& \frac{[(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}]}
 {[\xi t A_{ki,j}(s,\cos\phi_{1j})+(1-\xi) s A_{ki,j}(t,\cos\phi_{2j})][\xi t+(1-\xi)s]} \\
|M^{IIIa}|^2&=&g^4 S_\ep^2 \mu^{4 \ep} \frac{\hs_{ij}^2}{\tauN^4}\frac{s^2 t^2}{\xi^2(1-\xi)^2} 
         \Bigg[\frac{1}{A_{ki,j}(s,\cos\phiu) A_{ki,j}(t,\cos\phid)} \Bigg]\\
%
|M^{IIIb}|^2&=&-g^4 S_\ep^2 \mu^{4 \ep} \frac{\hs_{ij} \hs_{ik}}{\tauN^4}\frac{s^2 t^2}{\xi^2 (1-\xi)^2} 
  \Big(\frac{\big((\sqrt{s}-\sqrt{t})^2+4 \lambda \sqrt{st}\big)}{(s-t)^2} \Big) \nonumber \\
         &\times& \Bigg[\frac{1}{A_{ki,j}(s,\cos\phiu)}+\frac{1}{A_{ki,j}(t,\cos\phid)} \Bigg] \\
%
|M^{IIIc}|^2&=&g^4 S_\ep^2 \mu^{4 \ep} \frac{\hs_{ij} \hs_{ik}}{\tauN^4}\frac{1}{\xi (1-\xi)} \frac{s^3\; t^3}{2}
\frac{((\sqrt{s}-\sqrt{t})^2+4 \lambda \sqrt{st})}{(s-t)^2} \nonumber \\
         &\times& \Bigg[\frac{1}{\big(\xi t A_{ki,j}(s,\cos\phiu)+(1-\xi) s A_{ki,j}(t,\cos\phid)\big)\; (\xi t+(1-\xi) s)} \nonumber \\
    &\times & \Big(2+\frac{A_{ki,j}(s,\cos\phiu)}{ A_{ki,j}(t,\cos\phid)}+\frac{A_{ki,j}(t,\cos\phid)}{ A_{ki,j}(s,\cos\phiu)}\Big)\Bigg] \\
%
|M^{IIId}|^2&=&-g^4 S_\ep^2 \mu^{4 \ep} \frac{\hs_{ij}^2}{\tauN^4}\frac{s^3 t^3}{\xi (1-\xi)} \nonumber \\
         &\times& \Bigg[ \frac{1}{2 \; \big(\xi t A_{ki,j}(s,\cos\phiu)+(1-\xi) s A_{ki,j}(t,\cos\phid)\big)\; (\xi t+(1-\xi) s)}\nonumber \\
  &\times& \Big(\frac{1}{A_{ki,j}(s,\cos\phiu)}+\frac{1}{A_{ki,j}(t,\cos\phid)}\Big)\Bigg]
\eeqn
%Id,ansIIId=-Matfac*sij^2/tauN^4/xi/[1-xi]*s^2*t^2*(
%         s*t/2/[xi*t*Akij(s,cosphi1)+(1-xi)*s*Akij(t,cosphi2)]/[xi*t+(1-xi)*s] 
%         *(1/[Akij(s,cosphi1)]+1/[Akij(t,cosphi2)]));
%
\beqn
I^{(2),ij,I}_{q\bar{q},kk} &=& \cN_{ij} 2^{-6\ep} \big(\frac{\hs_{ik}}{\hs_{ij}}\big)^{2\ep}\;B_{RR} 
%\nonumber \\
%&&
\int_0^1  d\xi ds dt (\xi (1-\xi))^{1-2 \ep} \; (st)^{2+\ep} |s-t|^{-3-2\ep}\nonumber \\
&\times&\int_0^1 dx_4 \sin^{-2 \ep}\phiu
         \int_0^1 dx_5 \, (\lambda (1-\lambda))^{-\ep} 
         \times (-\ep) \int_0^1 \, d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
&\times& \frac{[ A_{ki,j}(s,\cos\phiu)- A_{ki,j}(t,\cos\phid)]^2\; [(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}]^{1+2 \ep}}
 {[\xi t A_{ki,j}(s,\cos\phiu)+(1-\xi) s A_{ki,j}(t,\cos\phid)]^2[\xi t+(1-\xi)s]^2}\nonumber \\
&\times& \theta(A_{ki,j}(s,\cos\phi_{1j})-s)\theta(A_{ki,j}(t,\cos\phi_{2j})-t)
\eeqn
This equation contains an apparent singularity as $s \to t$ that is in fact
regulated by the factor $[ A_{ki,j}(s,\cos\phiu)- A_{ki,j}(t,\cos\phid)]^2$,
as shown below.

Substituting in Eq.~(\ref{MsqII-case4}) we construct the equivalent of BLP, Eq~(24),  
\beqn
I^{(2),ij,II}_{q\bar{q},kk} &=& \cN_{ij} 2^{-6\ep} \big(\frac{\hs_{ik}}{\hs_{ij}}\big)^{2\ep}\;B_{RR} 
\frac{\hs_{ij}}{\hs_{ik}} \nonumber \\
&&\int_0^1  d\xi ds dt (\xi (1-\xi))^{-2 \ep} \; (st)^{1+\ep} |s-t|^{-1-2\ep}\nonumber \\
&\times&\int_0^1 dx_4 \sin^{-2 \ep}\phiu
         \int_0^1 dx_5 \, (\lambda (1-\lambda))^{-\ep} 
         \times (-\ep) \int_0^1 \, d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
&\times& \frac{[(\sqrt{s}-\sqrt{t})^2 +4 \lambda \sqrt{st}]^{2 \ep}}
 {[\xi t A_{ki,j}(s,\cos\phi_{1j})+(1-\xi) s A_{ki,j}(t,\cos\phi_{2j})][\xi t+(1-\xi)s]}\nonumber \\
&\times& \theta(A_{ki,j}(s,\cos\phi_{1j})-s)\theta(A_{ki,j}(t,\cos\phi_{2j})-t)
\eeqn
where $\cN$ is defined in Eq.~(\ref{Normalizationdefinition}).
Note that the symmetrization trick for $x_6$ only works if the integrand is a function only of $\sin\alphaud$,
which does not appear to be the case. Otherwise this equation looks pretty close to Eq.~(24) of BLP.

\beqn
I^{(2),ij,IIIa}_{q\bar{q},kk} &=& \cN_{ij} 2^{-4\ep} \big(\frac{\hs_{ik}}{\hs_{ij}}\big)^{2\ep}B_{RR}
\int_0^1  d\xi ds dt (\xi (1-\xi))^{-1-2 \ep} \; s^{\ep} \; t^{\ep}  \nonumber \\
 &\times & \int_0^1 dx_4 \sin^{-2 \ep}\phiu  \; \int_0^1 dx_5 \sin^{-2 \ep}\phid
         \times (-\ep) \int_0^1 \, d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
 &\times& \Big(\frac{\hs_{ij}}{\hs_{ik}}\Big)^2 \; \frac{1}{A_{ki,j}(s,\cos\phiu)\;A_{ki,j}(t,\cos\phid)} \nonumber \\
 &\times& \theta(A_{ki,j}(s,\cos\phi_{1})-s)\; \theta(A_{ki,j}(t,\cos\phi_{2})-t)
\eeqn
\beqn
I^{(2),ij,IIId}_{q\bar{q},kk} &=& \cN_{ij} 2^{-4\ep} \big(\frac{\hs_{ik}}{\hs_{ij}}\big)^{2\ep}B_{RR}
\int_0^1  d\xi ds dt (\xi (1-\xi))^{-2 \ep} \; s^{1+\ep} \; t^{1+\ep}  \nonumber \\
 &\times & \int_0^1 dx_4 \sin^{-2 \ep}\phiu  \; \int_0^1 dx_5 \sin^{-2 \ep}\phid
         \times (-\ep) \int_0^1 \, d x_6 \; x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
 &\times& \Big(\frac{\hs_{ij}}{\hs_{ik}}\Big)^2  \frac{1}
{2\; [\xi t A_{ki,j}(s,\cos\phiu)+(1-\xi) s A_{ki,j}(t,\cos\phid)] \, (\xi t+(1-\xi)s)}
\nonumber \\
&\times&\Big(\frac{1}{A_{ki,j}(s,\cos\phiu)}+\frac{1}{A_{ki,j}(t,\cos\phid)}\Big) \nonumber \\
 &\times& \theta(A_{ki,j}(s,\cos\phi_{1})-s)\; \theta(A_{ki,j}(t,\cos\phi_{2})-t)
\eeqn
where $\cN$ is defined in Eq.~(\ref{Normalizationdefinition}).
%
\subsubsection{The final sector decomposition}
We can write down the final result for part  of $ I^{(2),ij,II}_{q\bar{q},kk}$,
by performing a final separation,
\beq
1 = \theta(s-t)+\theta(t-s)
\eeq
For $s>t$,
\beq
\xi=x_1,\;\;  s=x_2,\;\; t=x_2(1-x_3),\;\;ds dt=x_2 dx_2 dx_3 
\eeq
\beqn
I^{(2),ij,II}_{q\bar{q},kk} &=& \cN_{ij} 2^{-6\ep} \big(\frac{\hs_{ik}}{\hs_{ij}}\big)^{2\ep}\;B_{RR} \frac{\hs_{ij}}{\hs_{ik}} \nonumber \\
&&\int_0^1  dx_1 dx_2 dx_3 dx_4 dx_5 dx_6 (x_1 (1-x_1))^{-2 \ep} \; x_2^{2\ep} (1-x_3)^{1+\ep} x_3^{-1-2\ep} \nonumber \\
&\times&\sin^{-2 \ep}\phiu
          \, (\lambda (1-\lambda))^{-\ep} 
         \times (-\ep) \, x_6^{-1-\ep}\; (1-x_6)^{-1-\ep} \nonumber \\
&\times& \frac{[(\sqrt{1}-\sqrt{1-x_3})^2 +4 \lambda \sqrt{1-x_3}]^{2 \ep}}
 {[x_1 (1-x_3) A_{ki,j}(x_2,\cos\phiu)+(1-x_1) A_{ki,j}(x_2(1-x_3),\cos\phid)][1-x_1x_3]}\nonumber \\
&\times& \theta(A_{ki,j}(x_2,\cos\phi_{1j})-x_2)\theta(A_{ki,j}(x_2(1-x_3),\cos\phi_{2j})-x_2(1-x_3))
\eeqn
This is to be compared with Eq.(28) of BLP.

The same transformation is applied to $I^{(2),ij,I}_{q\bar{q},kk}$.  In this
case it is useful to observe that, in the limit $x_3 \to 0$,
\beqn
&& \cos\phiud \to 1 - \frac{1-\lambda}{8\lambda} x_3^2 \,, \\
&& \sin\phiud \to \frac{\sqrt{1-\lambda}}{2\sqrt{\lambda}} x_3 \,.
\eeqn  
Hence,
\beqn
&& A_{ki,j}(s,\cos\phiu)- A_{ki,j}(t,\cos\phid) \nn \\
 &=& \frac{\hs_{ij}}{\hs_{ik}} x_2 x_3
  - 2 \sqrt{x_2 \frac{\hs_{ij} \hs_{jk}}{\hs_{ik}^2}}
  \left(\cos\phiu - \sqrt{1-x_3} \cos\phid \right) \nn \\
&=& \sqrt{x_2} \left[ \frac{\hs_{ij}}{\hs_{ik}} \sqrt{x_2} x_3
  - 2 \sqrt{\frac{\hs_{ij} \hs_{jk}}{\hs_{ik}^2}}
  \left(\cos\phiu(1-\sqrt{1-x_3} \cos\phiud)
   + \sqrt{1-x_3} \sin\phiu \sin\phiud\cos\alphaud \right) \right] \nn \\
&\to & x_3 \sqrt{x_2} \left[ \frac{\hs_{ij}}{\hs_{ik}} \sqrt{x_2}
  - \sqrt{\frac{\hs_{ij} \hs_{jk}}{\hs_{ik}^2}}
  \left(\cos\phiu
   + \sin\phiu \cos\alphaud \sqrt{\frac{1-\lambda}{\lambda}} \right) \right] \nn \\
\eeqn
using the relation, $\cos\phid=\cos\phiu \cos\phiud-\sin\phiu \sin\phiud\cos\alphaud$.

\color{black}

